Learning with Abandonment

Consider a platform that wants to learn a personalized policy for each user, but the platform faces the risk of a user abandoning the platform if she is dissatisfied with the actions of the platform. For example, a platform is interested in personalizing the number of newsletters it sends, but faces the risk that the user unsubscribes forever. We propose a general thresholded learning model for scenarios like this, and discuss the structure of optimal policies. We describe salient features of optimal personalization algorithms and how feedback the platform receives impacts the results. Furthermore, we investigate how the platform can efficiently learn the heterogeneity across users by interacting with a population and provide performance guarantees.

==> tex/basic.tex <==

\section{Model}


\subsection{Setup}

The general model we consider is as follows.
A single threshold $c$ is drawn from known distribution function $F$.
At time times $t=0,1,\ldots$, the platform sets activity level $x_t \in \mathbf{X}$,
where $\mathbf{X}$ is a given closed set.
While $x_t < c$, obtains a (random) reward of $R_t(x_t)$ with
expected value $\E(R_t(x_t)) = r(x_t) > 0$.
Let $T$ be the first time $x_t > c$: $T = \min\{\tau : x_\tau > c\}$.
The goal of the platform is to maximize the discounted sum of rewards up
to but not including the first crossing time $T$:
\[
  \max_{\{x_t\}} \E \left[ \sum_{t=0}^{T-1} \gamma^t R(x_t) \right],
\]
where $\gamma \in (0, 1)$ is the discount factor.
For convencience we write $S(\cdot) = 1 - F(\cdot)$ for the survival function.


\subsection{Optimal policy}

In this section, we take a deep dive into the baseline model.
We show that under general conditions there exists an optimal constant policy,
and it is easily characterized.
The proof is a straightfoward application of value iteration.

Besides the simplicity and generality of the result,
it is also noteworthy that the optimal policy does not depend on the discount factor.

\begin{theorem}
  Assume $r$ is positive for all $x \in \mathbb{X}$.
  Suppose the function $p: x \to r(x) S(x)$ has a unique global optimum at $x^*$.
  Then, the optimal policy is $x_t = x^*$ for all t, and the value is
  $r(x^*)S(x^*) / \gamma$.
\end{theorem}

\begin{proof}
  The proof follows from defining an appropriate dynamic program and
  solving it using value iteration.
  We will denote the state by $x$, denoting the best lower bound on $c$.
  In practice, if the process survives up to time $t$ ($T > t$)
  the state is $x = \max_{s \le t} x_s$.

  It is easy to see that the optimal policy is non-decreasing,
  so we can restrict our focus to non-decreasing policies.

  The Bellman equation for the value function at state $x$ is given by
  \[
  V(x) = \max_{y \ge x} \frac{S(y)}{S(x)} (r(y) + \gamma V(y)).
  \]
  For convenience we define the following transformation $ J(x) = S(x)V(x) $
  and note that we can equivalently use $J$ to find the optimal policy.
  We now explicitly compute the limit of value iteration to find $J(x)$.
  Start with $J_0(x) = 0$ for all $x$ and note that the iteration takes the form
  \[
      J_{k+1} = \max_{y \ge x} S(y) r(y) + \gamma J_k(y) = \max_{y \ge x} p(y) + \gamma J_k(y).
  \]
  We prove the following two properties by induction for all $k > 0$:
  \begin{enumerate}
    \item $J_k(x) = p(x^*) \sum_{i=0}^{k-1} \gamma_i$ for all $x \le x^*$.
    \item $J_k(x) < J_k(x^*)$ for all $x > x^*$.
  \end{enumerate}
  The above is immediately true for $k = 1$.
  Now assume it is true for an arbitrary $k$, then
  \[
  J_{k+1}(x) = p(x^*) + \gamma J_k(x^*) \qquad \text{ for all } x \le x^*
  \]
  and
  \[
  J_{k+1}(x) < p(x^*) + \gamma J_k(x^*) = J_{k+1}(x^*) \qquad \text{ for all } x > x^*.
  \]
  The result follows from taking the limit as $k \to \infty$ and noting that for any state $x \le x^*$,
  it is optimal to jump to state $x^*$ (and stay there).
  We also immediately see that the value of the optimal policy thus is $p(x) / \gamma$, as required.
\end{proof}

A key insight that is useful as we explore extensions to the model
is that the state of the dynamic program can be completely characterized
by the posterior over the threshold after observing survival up to time $t$
(i.e. $T > t$).
In the baseline model, this posterior is completely characterized by
the maximum activity level up to time $t$.

The intuition of the optimality of such a simple policy is also better understood from this perpective.
In a single time period, we are able to select exactly what subset of users (thresholds) we want to serve
to maximize rewards.
If, after an initial activity level of $x_0 = y$ for some $y$, it is better to set $x_1 = z > y$,
then we should have set $x_0 = z$ to begin with.

We note that the conditions for optimality of a constant policy are rather weak.
If $p$ has multiple global optima then any non-decreasing policy that jumps
between global optima of $p$ is optimal.


\subsection{Properties of optimal solution}

We now discuss properties of the optimal solution,
focusing on the case where the platform interacts with a user or agent.
The threshold $c$ models the user preference on when to abandon.

\subsubsection{Simple and widely applicable}
Practically speaking, the optimality of the constant policy has a number of advantages.
First of all, the result is widely applicable and barely relies on assumptions.
The policy is easily communicated to users,
and after a single time period users know whether they are happy or should abandon.

\subsubsection{Strategy-proof}

The proposed model implicitly assumes that agents are \emph{myopic}.
That is, the decision to abandon only depends on the current activity level.
Such agents fail to take into account how their decisions affect the actions of
the platform, and thus they might not act in their best interest.

In this section we show that the optimal policy is strategy-proof.
That is, also for \emph{strategic} (or rational) agents
the same constant policy is optimal.
To do this, we draw a parallel to the viewpoint of mechanism design.

The idea is to relax the constraint that there is permanent abandonment and
find an optimal mechanism for setting activity levels.
It turns out that this leads to the a policy that is also optimal in the
constraint case, and equivalent to the solution based on dynamic programming.

\begin{prop}
  Assume $r$ is positive for all $x \in \mathbb{X}$.
  Suppose the function $p: x \to r(x) S(x)$ has a unique global optimuum at $x^*$.
  The constant policy $x_t = x^*$ is an optimal policy for strategic agents.
\end{prop}

\begin{proof}
By the revelation principle \cite{myerson1981optimal} suppose the principal
queries the agent for her threshold $\tilde c$,
and implements the allocation rule $x_t(\tilde c)$.
The goal of the principal is to maximize her total discounted reward.
\[
  \max \sum \gamma^t r(x_t(\tilde c))
\]
under incentive compatibility and individual rationality constraints.
For now, we relax the problem by forgetting about the abandonment constraint.
We want to design a mechanism that maximizes the reward over allocation rules
$x_t(\tilde c)$.

The (scaled) total discounted utility for the consumer is
\[
  (1-\gamma) \sum_{t=0}^\infty \gamma^t (c - x_t( \tilde c))
    = c - (1-\gamma) \sum_{t=0}^\infty \gamma^t x_t(\tilde c)
    = c - q(\tilde c)
\]
where we implicitly define $q$ as the cost of the allocation schedule to the
agent.
But this is exactly the monopoly pricing problem and we know that posted prices
are optimal.
That is, the principal implements $x_t = z$ if $\tilde c \ge z$ and $x_t = 0$
otherwise, for all time steps $t$, for some $z$.
This satisfies the incentive compatibility and individual rationality
constraints.
Moreover, we note that this also adheres to the specific condition that
$x_t = 0$ for all $t > s$ if $x_s > c$.
we note that the solution also adheres to the condition that the agent can only
switch once and for all to the alternative with utility $0$.
To maximize the total discounted reward, the principal selects $z$ to maximizes
\[
  \max_z r(z) S(z).
\]
Hence, the optimal mechanism is equal to the optimal policy.
\end{proof}




% \subsection{Assumptions}

% A list with assumptions that we use throughout the work.

% \begin{assumption}[non-negative reward]
%   \label{ass:rnneg}
%   Reward function $r$ is non-negative, i.e. $r(x) \ge 0$ for all $x \in \X$.
% \end{assumption}

% \begin{assumption}[non-decreasing reward]
%   \label{ass:rndec}
%   The reward function $r$ is non-decreasing, i.e. $r(y) \ge r(x)$ for all $y > x$.
% \end{assumption}

% \begin{assumption}[Lipschitz reward]
%   \label{ass:rlip}
%   The reward function is $L$-Lipschitz, i.e. $|r(y) - r(x)| \le L|y - x|$ for
%   all $x, y$.
% \end{assumption}

% \begin{assumption}[bounded reward]
%   \label{ass:rbdd}
%   The reward function is upper bounded by $B$, i.e. $r(x) \le B$ for all $x \in \X$.
% \end{assumption}



==> tex/main.tex <==
\title{Learning with abandonment}
\author{Ramesh Johari and Sven Schmit}
\date{\today}

\begin{document}

    \maketitle
    \input{tex/abstract}


    \input{tex/intro}
    \input{tex/model}
    \input{tex/feedback}

    % \input{tex/signals}

    \input{tex/learning}
    \input{tex/conclusion}


    \bibliographystyle{plainnat}
    \bibliography{bib/bibliography}

\end{document}


==> tex/related.tex <==
\section{Related work}

\subsection{Dynamic pricing}
No repeat transactions; customers interact once and price can be ajusted over time.

\citet{rothschild1974two} considers learning the demand curve of a product
using a multi-armed bandit approach.
The work assumes that customers arrive only once,
and it is therefore not possible to learn about specific users.


\citet{farias2010dynamic} give an overview on dynamic pricing and consider
a setting where there is an initial inventory $x_0$ that gets sold over time and
the merchant is able to dynamically adjust prices $p(t)$.
They consider the case where customers arrive according to a Poisson process with
unknown arrival rate and their reservation price is drawn from a distribution $F$.

\subsection{Dynamic mechanism design}
There is a vast literature on mechanism design where the principal
designs pricing and allocation mechanism to sell a single or multiple goods,
starting by the work \cite{myerson1981optimal}.
Recently, there has been a flurry of interest in the dynamic case,
where at each time $t=1,2,\ldots$ a good is sold \cite{pavan2014dynamic, bergemann2010dynamic,
  Kakade2013OptimalDM, Skrzypacz2014MechanismsFR, athey2013efficient}.
This leads to interesting dynamics such as commitment problems
\cite{lobel2017dynamic} when information arrives over time.
There are two key differences between this line of research and our work.
First, our main focus is not on strategic agents, but on agents using simpler
heuristics, though we do mention where this leads to differences.
The second difference is that the setting of a single user that abandons
the principle forever has not been studied.
This can partly be explained by the fact that this might not be optimal from a
strategic agent's perspective; or it can be viewed as a severe restriction on
the action space of agents.

\subsection{Revenue management}

\citet{gallego1994optimal} considers the problem of selling a given stock of
items by a deadline with non-strategic agents; these do not take into account
future changes in price, and show that constant pricing policies are
asymptotically optimal.


There has been work on pricing under uncertainty, such as
\cite{bergemann2008pricing, bergemann2011robust, parakhonyak2015non,
caldentey2016intertemporal}.
Roughly speaking, we see that prices are lowered under uncertainty.


Partial monitoring?

Safe reinforcement learning?

Planning problems?





